The 2019 Taurid resonant swarm: prospects for ground detection of small NEOs

In June 2019 the Earth will approach within 5{\deg} mean anomaly of the centre of the Taurid resonant swarm, its closest post-perihelion encounter with Earth since 1975. This will be the best viewing geometry to detect and place limits on the number of NEOs proposed to reside at the swarm centre until the early 2030s. We present an analysis of the optimal times and pointing locations to image NEOs associated with the swarm

==> Removals.tex <==
Fig.~\ref{Fig:MagAndMotion} plots all TS object sky motion an magnitudes by date throughout the TS passage, with three viewing opportunities (labeled A, B), and a motion-magnitude area of interest labelled C), suggested by inspection of in-sky motion, apparent magnitudes, and occurrences of a full moon on 2019/06/17 (JD~2458651.5), 2019/07/16 (JD~2458680.5), and  2019/08/15 (JD~2458710.5). Periods of 5 days on either side of a full moon are shaded as less favourable. Refer to Table~\ref{Tab:Calendar} for a summary of all relevant dates.  Opportunities A and B correspond to two date ranges over which observing campaigns may be successful in detecting $H=24$ objects.  Area C of the plot highlights the time span between June and July full moons where many bright fast moving objects are present but are likely moving too fast for sidereal tracking and positive object detection.

This target area is close to the galactic plane, but {\color{red} {Need to be specific,supported by images?)}} sufficiently far from both the plane and galactic center so as to not me saturated with background objects.
